GupShup: An Annotated Corpus for Abstractive Summarization of Open-Domain Code-Switched Conversations

Code-switching is the communication phenomenon where speakers switch between different languages during a conversation. With the widespread adoption of conversational agents and chat platforms, code-switching has become an integral part of written conversations in many multi-lingual communities worldwide. This makes it essential to develop techniques for summarizing and understanding these conversations. Towards this objective, we introduce abstractive summarization of Hindi-English code-switched conversations and develop the first code-switched conversation summarization dataset - GupShup, which contains over 6,831 conversations in Hindi-English and their corresponding human-annotated summaries in English and Hindi-English. We present a detailed account of the entire data collection and annotation processes. We analyze the dataset using various code-switching statistics. We train state-of-the-art abstractive summarization models and report their performances using both automated metrics and human evaluation. Our results show that multi-lingual mBART and multi-view seq2seq models obtain the best performances on the new dataset

==> defpack.tex <==

\usepackage[utf8]{inputenc} % allow utf-8 input
\usepackage[T1]{fontenc}    % use 8-bit T1 fonts
\usepackage{hyperref}       % hyperlinks
%\usepackage{url}            % simple URL typesetting
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{microtype}      % microtypography
\usepackage{cite}
\usepackage{xcolor}
\usepackage{framed}
\colorlet{shadecolor}{pink}
\usepackage{authblk}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{graphicx}
\usepackage{soul}
\usepackage{subcaption}
\usepackage{booktabs} % for professional tables
\usepackage{tablefootnote}
\newcommand{\theHalgorithm}{\arabic{algorithm}}

\usepackage{amsmath,amsthm,amssymb,amsfonts}
\usepackage{algorithm}
\usepackage{algorithmic}
\usepackage{enumerate}
\usepackage{cleveref}
\usepackage{comment}
\usepackage{bm}
\usepackage{pifont}
\newcommand{\cmark}{\ding{51}}%
\newcommand{\xmark}{\ding{55}}%

\theoremstyle{plain}
\newtheorem{theorem}{Theorem}[]
\newtheorem{corollary}{Corollary}[theorem]
\newtheorem{lemma}[]{Lemma}
\newtheorem{proposition}{Proposition}

%\theoremstyle{definition}
\newtheorem{definition}{Definition}[]
\newtheorem{assumption}{Assumption}[]

%\theoremstyle{remark}
\newtheorem{remark}{Remark}[]

\newcommand{\ra}[1]{\renewcommand{\arraystretch}{#1}}
\renewcommand{\qedsymbol}{$\blacksquare$}

\def\x{{\mathbf x}}
\def\z{{\mathbf z}}
\def\a{{\mathbf a}}
\def\A{{\mathbf A}}
\def\P{{\mathbf P}}
\def\r{{\mathbf r}}
\def\s{{\mathbf s}}
\def\u{{\mathbf u}}
\def\y{{\mathbf y}}
\def\I{{\mathbf I}}
\def\e{{\boldsymbol{\nu}}}
\def\Rb{{\mathbb{R}}}
\def\C{{\mathbf C}}

\def\G{{\mathcal G}}
\def\E{{\mathbb E}}
\def\O{{\mathcal O}}
\def\R{{\mathbb{R}}}

\newcommand{\ts}{\textsuperscript}
\newcommand{\highlight}[1]{%
  \colorbox{yellow!100}{$\displaystyle#1$}}
